The Grand Illusion: The Myth of Software Portability and Implications for ML Progress

Pushing the boundaries of machine learning often requires exploring different hardware and software combinations. However, the freedom to experiment across different tooling stacks can be at odds with the drive for efficiency, which has produced increasingly specialized AI hardware and incentivized consolidation around a narrow set of ML frameworks. Exploratory research can be restricted if software and hardware are co-evolving, making it even harder to stray away from mainstream ideas that work well with popular tooling stacks. While this friction increasingly impacts the rate of innovation in machine learning, to our knowledge the lack of portability in tooling has not been quantified. In this work, we ask: How portable are popular ML software frameworks? We conduct a large-scale study of the portability of mainstream ML frameworks across different hardware types. Our findings paint an uncomfortable picture -- frameworks can lose more than 40% of their key functions when ported to other hardware. Worse, even when functions are portable, the slowdown in their performance can be extreme and render performance untenable. Collectively, our results reveal how costly straying from a narrow set of hardware-software combinations can be - and suggest that specialization of hardware impedes innovation in machine learning research.

==> Figures/tables_timings/gpu_top5.tex <==
\begin{table}
\centering
\caption{Comparison of the latency in milliseconds for top two biggest and least slow down functions in TensorFlow, PyTorch, and JAX on GPU and TPU. The table is ordered by relative difference - (TPU - GPU)/GPU - in descending order, and the top two biggest slow down functions are highlighted. Note that the Latency on GPU and TPU values are rounded to 6 decimal places, and the relative difference is rounded to 2 decimal places.}
\vspace{1em}
\label{tab:test}
\begin{tabular}{l l r r r}
\toprule
    &  Function &  GPU &  TPU &  (TPU - GPU)/GPU \\
\midrule
TensorFlow & \cellcolor{gray!15}tf.linalg.svd & \cellcolor{gray!15}0.000931 & \cellcolor{gray!15}0.112843 & \cellcolor{gray!15}120.21 \\
    & \cellcolor{gray!15}tf.math.reduce\_logsumexp & \cellcolor{gray!15}0.013028 & \cellcolor{gray!15}0.474586 & \cellcolor{gray!15}35.43 \\
    & tf.estimator.LoggingTensorHook & 0.000042 & 0.000038 & -0.10 \\
    & tf.compat.v1.Session.run & 0.005722 & 0.003804 & -0.34 \\
\midrule
PyTorch  & \cellcolor{gray!15}torch.argsort & \cellcolor{gray!15}0.000157 & \cellcolor{gray!15}0.948210 & \cellcolor{gray!15}6038.55 \\
    & \cellcolor{gray!15}torch.optim.Adamax & \cellcolor{gray!15}0.000069 & \cellcolor{gray!15}0.392712 & \cellcolor{gray!15}5690.48 \\
    & torch.cuda & 0.000041 & 0.000061 & 0.49 \\
    & torch.nn.Conv2d & 0.046053 & 0.067081 & 0.46 \\
\midrule
JAX & \cellcolor{gray!15}jax.named\_call & \cellcolor{gray!15}0.000007 & \cellcolor{gray!15}0.000012 & \cellcolor{gray!15}0.71 \\
    & \cellcolor{gray!15}jax.numpy.array & \cellcolor{gray!15}0.000435 & \cellcolor{gray!15}0.000638 & \cellcolor{gray!15}0.47 \\
    & jax.numpy.cos & 0.172002 & 0.026102 & -0.85 \\
    & jax.numpy.sqrt & 0.098118 & 0.013860 & -0.86 \\
\bottomrule
\end{tabular}
\end{table}

 % \dzung{TensorFlow is without soft replacement. NOTE: I remove the failures from this chart. For example, if a test passes on the GPU but fails on the TPU, it will not be calculated for the average}

==> Figures/tables_timings/tpu_top5.tex <==
\begin{table}
\centering
\caption{}
\label{tab:tpu_top5}
\begin{tabular}{lllrrr}
\toprule
    &   &            Function &  Latency on GPU &  Latency on TPU &  (GPU - TPU)/TPU \\
\midrule
\textbf{TensorFlow} & 1 &         simple\_save &        0.199838 &        0.048309 &             3.14 \\
    & 2 &                 run &        0.005475 &        0.003653 &             0.50 \\
    & 3 &                eval &        0.003318 &        0.003311 &             0.00 \\
    & 4 &      list\_variables &        0.000507 &        0.000521 &            -0.03 \\
    & 5 &      get\_collection &        0.000006 &        0.000008 &            -0.25 \\\midrule
\textbf{PyTorch} & 1 &              conv2d &        0.046053 &        0.068429 &            -0.33 \\
    & 2 &                cuda &        0.000041 &        0.000062 &            -0.34 \\
    & 3 &  register\_parameter &        0.000039 &        0.000098 &            -0.60 \\
    & 4 &       concatdataset &        0.000031 &        0.000105 &            -0.70 \\
    & 5 &             Dataset &        0.000035 &        0.000152 &            -0.77 \\\midrule
\textbf{JAX} & 1 &                sqrt &        0.098118 &        0.013860 &             6.08 \\
    & 2 &                 cos &        0.172002 &        0.026102 &             5.59 \\
    & 3 &             PRNGKey &        1.485077 &        0.227995 &             5.51 \\
    & 4 &             one\_hot &        0.138935 &        0.023335 &             4.95 \\
    & 5 &                  ge &        0.090087 &        0.015302 &             4.89 \\
\bottomrule
\end{tabular}
\end{table}

